Conditional Diffusion Models for Weakly Supervised Medical Image Segmentation

Recent advances in denoising diffusion probabilistic models have shown great success in image synthesis tasks. While there are already works exploring the potential of this powerful tool in image semantic segmentation, its application in weakly supervised semantic segmentation (WSSS) remains relatively under-explored. Observing that conditional diffusion models (CDM) is capable of generating images subject to specific distributions, in this work, we utilize category-aware semantic information underlied in CDM to get the prediction mask of the target object with only image-level annotations. More specifically, we locate the desired class by approximating the derivative of the output of CDM w.r.t the input condition. Our method is different from previous diffusion model methods with guidance from an external classifier, which accumulates noises in the background during the reconstruction process. Our method outperforms state-of-the-art CAM and diffusion model methods on two public medical image segmentation datasets, which demonstrates that CDM is a promising tool in WSSS. Also, experiment shows our method is more time-efficient than existing diffusion model methods, making it practical for wider applications.

==> subsection/intro_v2.tex <==
Self-supervised contrastive learning \cite{chen2020simple,chen2020mocov2,grill2020bootstrap,chen2021exploring} has made strides over traditional self-supervised pretexts tasks  \cite{zhang2016color,noroozi2016jigsaw,gidaris2018unsupervisedrot} in natural scene representation learning.
However, the jury is still out for whether this is true for biomedical imaging (BMI) despite recent contrastive works \cite{Azizi2021BigSM,Chaitanya2020ContrastiveLO,Sowrirajan2021MoCoPI}.
A key hindrance involves the sub-optimal selection of "similar" and "dissimilar" images (we refer to these image sets as \emph{positives} and \emph{negatives}, respectively).
Natural scene contrastive learning uses instance discrimination where features extracted from transformed versions of the same images are positives and made similar while the features of negatives, which contain all other image instances, are contrasted.
As a result, two different images that contain similar content are erroneously treated as negatives.
% while simultaneously passing the chance to learn more robust representations of the same image pair.
This drawback is stifled in natural scene datasets in part because of large numbers of categories, diverse appearances within as well as between categories, and the sheer volume of unlabeled data present.
However, the same cannot be said in BMI tasks, especially BMI segmentation datasets, which contain fewer semantic categories, comparably homogeneous appearances, fewer data instances, and problematic class imbalances.
% Instance-level contrasting is better suited for natural scene images (NSIs) as opposed to biomedical images (BMIs) since NSIs contain more semantic categories (benchmarked in thousands), diverse appearances within as well as between categories (as opposed to more visual homogeneity in BMIs), and benefit from larger datasets (compared with smaller BMI data due to confidentially, acquisition, and cost hurdles). 
% The core idea stems from metric learning in that feature distances between "similar" or \emph{positive} images should be small while features of "contrasting" or \emph{negative} images should be distant.

Recent contrastive learning methods for BMI segmentation address these instance discrimination drawbacks and propose improved selection methods of positives and negatives. 
Azizi et al. \cite{Azizi2021BigSM} and Vu et al. \cite{Vu2021MedAugCL} both show improvements over instance discrimination baselines by expanding positives to all images from the same patient.
However, this approach relies on the availability of medical meta-data and multiple scans per patients which isn't widely guaranteed.
Instead of depending upon meta-data, LGCL \cite{Chaitanya2020ContrastiveLO} and PCL  \cite{zeng2021positional} make use of 3D spatial priors by hypothesizing that slices with corresponding axial positions contain semantically similar anatomical structures.
Thus, positives can be defined as images within similar spatial positions while negatives can be finely tuned based on the expected semantic overlaps.
These methods make the assumption of reasonable image pre-alignment and, although they operate in planar slices, cannot be applied to generic 2D tasks.


In order to develop a more general method, we seek to define image similarity by clustering features extracted in an unsupervised manner.
This then begs the paradoxical question, how do we effectively retrieve these features if learning good features is the task in the first place?
Give choices here, and justificiations.
Previously, \cite{zheng2019biomedical} also make use of auto-encoders to cluster features in an unsupervised manner. 
They use this principle for improved sample selection for label efficiency.


In this paper, we propose a novel cluster-guided contrastive learning framework (nicknamed CGC(?)) that outperforms instance discrimination pretraining, and works generally across BMI modalities \& tasks without relying on prerequisite meta-data, availability of additional views, or alignment assumptions. 
In the first stage, categorical information is extracted from all unlabaled data in an unsupervised manner by hierarchically clustering features learned by a variational auto-encoder (VAE).
In stage two, we pretrain a convolutional encoder with contrastive learning that's guided by pseudo-categories from stage one clustering results to select positives and negatives.
Finally, we transfer the encoder to fine-tune on a downstream segmentation task to evaluate the quality of features learned. 
We evaluate our framework on a skin lesion segmentation task and a heart CT segmentation dataset (MMWHS). 
The results show that our method outperforms state-of-the-art baselines in both semi-supervised and transfer learning settings.

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table*}[t]
    %\small
    %\footnotesize
    \scriptsize
    \centering
    \caption{Comparisons between state-of-the-art methods and the proposed methods w.r.t. segmentation dice scores on multi-organ segmentation dataset (Synapse). The last three rows are our proposed methods, and SimPROT-W means SimPROT pre-training with attention weight $w=5$ in the loss function.}
    \label{table1}
    \begin{tabularx}{\linewidth}{C|YYY|YYY}
    \toprule
\multirow{2}{*}{Methods}  & \multicolumn{3}{c|}{\textbf{BraTs flair}}   & \multicolumn{3}{c}{\textbf{CHAOS}} \\ \cline{2-7}
% & $0.05*|X_{tr}|$  & $0.1*|X_{tr}|$ & $0.2*|X_{tr}|$ & $0.1*|X_{tr}|$  & $0.2*|X_{tr}|$ & $0.4*|X_{tr}|$  \\
 &\multicolumn{1}{c}{Dice} & \multicolumn{1}{c}{mIoU} & \multicolumn{1}{c|}{hd} & \multicolumn{1}{c}{Dice}  & \multicolumn{1}{c}{mIoU} & \multicolumn{1}{c}{hd} \\
 \hline

 
UNETR   &84.61  &82.94  &83.62  &55.42    &93.09  &68.45   \\
 
 \hline
Swin UNETR  &88.26 &84.22 &85.91 &61.63 &94.81 & 77.94  \\


\hline
supervised & 0.914(0.058) & 0.847(0.093) & 8.093(11.879) & 0.914$\pm$0.058 & 0.847$\pm$0.093 & 8.093$\pm$11.879    \\

% \midrule[1pt]
% \multicolumn{1}{c}{benchmark} & \multicolumn{3}{c}{  0.878  (full $|X_{tr}|$)}                        & \multicolumn{3}{l}{}      \\
\bottomrule
\end{tabularx}
    
\end{table*}

==> subsection/related_works.tex <==
\textbf{Domain Adaptation for semantic segmentation}
% general application and medical application
Domain adaptation is a sub-problem of transfer learning, where the difference of the two problems is due to data being collected from different datasets. In this paper, we only focus on the unsupervised domain adaptation on semantic segmentation.
One straightforward solution to this problem is training the model to learn domain-independent features. 
\cite{luo2019taking} added two classifiers to the encoder in order to get diverse view for a feature, and they extended traditional adversarial loss with an adaptive loss, which was calculated by the cosine distance between the output of those two classifiers. 
Therefore, the follow-up discriminator would focus more on poorly aligned categories.
Instead of using adversarial learning, \cite{zhang2019category} tried to aggregate features belonging to the same categories for different domain images. Since they did not have annotation for the target domain images, they used a model pretrained on the source domain to generate pseudo-labels.
% The above works both focus on city-view images, like CITYpass.
\cite{ouyang2019data} fused prior matching to a VAE model to learn a shared feature space between two domains. 
More specifically, two domains had a shared VAE module and distinct encoder and decoder modules, and they applied adversarial learning to align features extracted from different encoders.
The work\cite{wu2021unsupervised} was also based on VAE but did not directly decrease the discrepancy of latent features for both domains. 
Instead, they drove the distribution of feature maps to the same parameterized variational form. 

Image translation is an alternative way to tackle UDA. Compared to feature alignment in latent space, we can just generate images out of an existing dataset that shares a similar distribution as another dataset. After that, we can take advantage of the annotated domain to do supervised training.
The feasibility is ascribed to the rapid development of generative adversarial model (GAN), especially the emergence of CycleGAN\cite{zhu2017unpaired} in unpaired image translation. 
\cite{hoffman2018cycada} firstly integrated a segmentation model with the CycleGAN module for road scene images from different sources.
% They actually also added feature adaptation loss for the training, but they did not include the real target domain images in the cycle.
At the same time, \cite{huo2018adversarial} used the integrated framework to achieve domain adaptation on CT-MR abdomen segmentation.
SIFA\cite{chen2020unsupervised} further extended the workflow by making the segmenter and the source domain generators share the encoder, adding a discriminator to the segmentation results as well as the latent embedding in generated image space.
Most recently, \cite{tomar2021self} proposed to add an attention mechanism in the form of normalization to features in the generator to improve the quality of synthesized images for SIFA.

\textbf{Contrastive learning}
Previously, there were already several works exploring representation learning in an unsupervised way as pretext task, including context prediction\cite{pathak2016context}, colorization\cite{larsson2017colorization}, and rotation prediction\cite{gidaris2018unsupervised}.
Contrastive learning gained popularity after the work SimCLR\cite{chen2020simple}. 
The basic idea is that original image and its augmentations should be the same in the latent space, and this pretext task can boost the performance for the downstream classification task.
Even with a simple linear classifier, SimCLR could reach competitive performance on a large scale dataset.
Follow-up works provided different perspectives of influential factors, such as transformation combinations\cite{chen2020big}, batch size and momentum encoders\cite{he2020momentum, chen2021exploring}, as well as supervised class clustering\cite{khosla2020supervised}. 
Due to the powerful ability of representation learning, this emergent technique has been applied to other areas.
CUT\cite{park2020contrastive} first used contrastive learning for image synthesis .
They tried to maximize the mutual information between patches from the same position for the original and generated images so that the content remained unchanged after translation.
\cite{chaitanya2020contrastive, zeng2021positional} observed the similarity of adjacent slices in 3D medical image scans and explored how this kind of knowledge could improve the segmentation performance with less labeled data.
